Offline Vehicle Routing Problem with Online Bookings: A Novel Problem Formulation with Applications to Paratransit

Vehicle routing problems (VRPs) can be divided into two major categories: offline VRPs, which consider a given set of trip requests to be served, and online VRPs, which consider requests as they arrive in real-time. Based on discussions with public transit agencies, we identify a real-world problem that is not addressed by existing formulations: booking trips with flexible pickup windows (e.g., 3 hours) in advance (e.g., the day before) and confirming tight pickup windows (e.g., 30 minutes) at the time of booking. Such a service model is often required in paratransit service settings, where passengers typically book trips for the next day over the phone. To address this gap between offline and online problems, we introduce a novel formulation, the offline vehicle routing problem with online bookings. This problem is very challenging computationally since it faces the complexity of considering large sets of requests -- similar to offline VRPs -- but must abide by strict constraints on running time -- similar to online VRPs. To solve this problem, we propose a novel computational approach, which combines an anytime algorithm with a learning-based policy for real-time decisions. Based on a paratransit dataset obtained from the public transit agency of Chattanooga, TN, we demonstrate that our novel formulation and computational approach lead to significantly better outcomes in this setting than existing algorithms.

==> GreedyAlgoDir/Reachable.tex <==
\begin{algorithm}[!h]
 \caption{$\textbf{Reachable}(l_1, w_1, l_2, w_2, D^{\textit{dwell}})$}
 \label{algo:reachable}
        
$\textit{reachable} \leftarrow w_1^{\textit{start}} + D^{\textit{travel}}_{l_1,l_2} + D^{\textit{dwell}} \leq w_2^{\textit{end}}$
        
\KwResult{reachable}
\end{algorithm}

==> sub/anytime_model.tex <==
\paragraph{Extended PDPTW Problem Model}
We represent the overall system by a graph G = $(\mathcal{Y}, \mathcal{E})$, where $\mathcal{Y}$ is a set of vertices and $\mathcal{E}$ is a set of \ad{directional?} edges. Each edge connects a pair of nodes as long as the edge contains a feasible drive without violating the travel-time and time-window constraints\Aron{it is not specified anywhere which nodes are connected by edges (I'm assuming that there exists an edge for any feasible drive, i.e., for any pair of nodes where travel times is less than difference between earliest time at origin and latest time at destination)}. We use \textit{nodes} and \textit{vertices} interchangeably. The pickup and dropoff locations for each request are represented by \textit{unique} nodes in the graph. In other words, if multiple requests originate from or terminate at the same geographic location, they are represented as separate nodes in the graph. We associate a time-window with each pick-up node; for example, the pickup location for request $r_i \in \mathcal{R}$ has the pick-up time window $[a^{i}, b^{i}]$ associated with it. This window denotes that some vehicles need to visit the pick-up node within the time limits specified by the associated window.

We also add two special nodes to the graph known as \textit{depots}. Depots are analogous to source and sink nodes in classical formulations dealing with the vehicle routing problem. In such formulations, source and sink nodes are virtual and do not correspond to actual physical locations. Depots can also be used to denote stations where vehicles are housed. We assume that each depot has enough capacity to house all the vehicles. 

We use $\mathcal{N}^{p}$, $\mathcal{N}^{d}$, and $\mathcal{N}^{s}$  to denote the set of all the pick-up nodes, drop-off nodes, and depots (source and sink nodes) respectively. We also use $\mathcal{N}^{ab}$ to denote the union of arbitrary sets $\mathcal{N}^{a}$ and $\mathcal{N}^{b}$. For example, $\mathcal{N}^{pd} = \mathcal{N}^{p} \cup \mathcal{N}^{d}$ indicates set of all the pickup and dropoff nodes. 


==> sub/constraints.tex <==
\paragraph{Decision Variables}
We use the following decision variables to formulate the problem. $x_{i,j}^m \in \{0,1\}$ --- if the route $m \in \mathcal{M}$ \ad{should state that we assume routes are a indexed by a set of positive integers}\Aron{we don't need this assumption} is assigned to drive the edge connecting the nodes $i, j \in \mathcal{N}$ then $x^m_{i,j} = 1$, otherwise $x^m_{i,j} = 0$. Note that while we formulate the problem in terms of variables assigned to paths, the variables implicitly define an optimization problem over nodes. Specifically, if a route is assigned to an edge from a pickup node, then the constraints (defined below) ensure that it must pickup the passenger from the said node. $t^i \in \mathbb{Z}^{+}$ --- indicates the time when an assigned vehicle reaches the location $i \in \mathcal{N}$. $o^i \in \mathbb{Z}^{+}$ --- indicates the occupancy when vehicle leaves the location $i \in \mathcal{N}$. $s^m \in \mathbb{Z}^{+}$ --- indicates the start time of the route $m \in \mathcal{M}$. $e^m \in \mathbb{Z}^{+}$ --- indicates the end time of the route $m \in \mathcal{M}$.
\ad{we should make it clear that there are two decision points. First, determining the route that will serve a node. Second determining the vehicle that will serve the route}
\paragraph{Constraints}
The extended PDPTW problem needs to ensure the constraints listed below,
{\scriptsize
\begin{align}
    &\sum_{m \in \mathcal{M}} ~  \sum_{n'\in \Delta^{+}(n)} ~ x^m_{n, n'} = 1 \;\;\;\; \forall{n \in \mathcal{N} \setminus \mathcal{N}^s}
    \label{eqn:assign_constraint}\\&\sum_{d \in \mathcal{N}^s} \sum_{n \in \mathcal{N}^{p}} x^m_{d, n} = 1\;\;\;\; \forall{m \in \mathcal{M}} \label{eqn:start_from_depot_constraint}\\&\Big(\sum_{j \in \mathcal{N}} x^m_{j,i} - \sum_{k \in \mathcal{N}} x^m_{i,k}\Big)= 0 \;\;\;\; \forall{m \in \mathcal{M}} \;\;\;\; \forall{i \in \mathcal{N}^{pd}} \label{eqn:flow_constraint}\\&\Big(\sum_{j \in \mathcal{N}^{pd}} x^m_{p_i,j} - \sum_{k \in \mathcal{N}^{pd}} x^m_{k,d_i}\Big) = 0 \;\;\;\;\forall{m \in \mathcal{M}} \;\;\;\; \forall{r_i \in \mathcal{R}}\label{eqn:same_vehicle_constraint}
    \\&\textbf{If $x^m_{i,j} = 1$} \nonumber\\
    & \;\;\;\; t^{i} - t^{j} + T_{i,j} + \tau_{d} \leq 0 \;\;\;\; \forall{i,j \in \mathcal{N}} \;\;\;\; \forall{m \in \mathcal{M}}
    \label{eqn:time_limit_constraint}\\& \;\;\;\; s^m - t_j + T_{i,j} \leq 0 \;\;\;\; \forall i \in \mathcal{N}^s \;\;\;\; \forall j \in \mathcal{N}^{p} \;\;\;\; \forall m \in \mathcal{M}
    \label{eqn:time_limit_constraint_f_start}\\& \;\;\;\; t^i + T_{i,j} + \tau_{d} - e^m \leq 0 \;\;\;\; \forall i \in \mathcal{N}^{d} \;\;\;\; \forall j \in \mathcal{N}^{s} \;\;\;\; \forall m \in \mathcal{M}
    \label{eqn:time_limit_constraint_f_end}\\&a^i \leq t^{p_i} \leq b^i \;\;\;\; \forall r_i \in \mathcal{R}\label{eqn:pick_up_time_window}\\&a^i + T_{p_i,d_i} \leq t^{d_i} \leq b^i + T_{p_i,d_i} + \tau_s \;\;\;\; \forall r_i \in \mathcal{R}\label{eqn:drop_off_time_window}\\& e^m - s^m
   \leq \tau_{max} \;\;\;\; \forall{m \in \mathcal{M}}
    \label{eqn:operation_constraint_t_short}\\&o^{p^j} = \left(\sum_{m \in \mathcal{M}}\sum_{i \in \mathcal{N}} \left\{x^m_{i,j} \cdot o^{i} \right\} \right)  + c_j \leq C \;\;\;\;\forall{r_j \in \mathcal{R}}\label{eqn:capacity_constraint_a}\\&0 \leq o^{d^j} = \left(\sum_{m \in \mathcal{M}}\sum_{i \in \mathcal{N}}\left\{x^m_{i,j} \cdot o^{i} \right\} \right) - c_j \;\;\;\;\forall{r_j \in \mathcal{R}}\label{eqn:capacity_constraint_b}\\&o^{k} = 0\;\;\;\;\forall{k \in \mathcal{N}^{s}} \label{eqn:capacity_constraint_ss}\\ &\sum_{v \in \mathcal{V}} y^v_{m} \leq 1 \;\;\;\;  \forall{m \in \mathcal{M}} \label{eqn:run_assignment}
\end{align}
}

First, we look into general constraints related to the assignment of requests to routes. The \cref{eqn:assign_constraint} ensures only one route can serve an edge connecting two locations $n,n' \in \mathcal{N}$, where $\Delta^{+}(n)$ contains the set of immediate nodes which can be reached from the node $n$ during the flow.  Note that the function $\Delta^{+}(n)$ generates feasible nodes during the preprocessing stage by considering time constraints. The \cref{eqn:start_from_depot_constraint,eqn:assign_constraint,eqn:flow_constraint} ensure each route $m \in \mathcal{M}$ starts serving requests from a depot and returns back to a depot. The \cref{eqn:flow_constraint} ensures each route $m \in \mathcal{M}$ that visits a pickup, or a dropoff node must leave the node. The \cref{eqn:same_vehicle_constraint} ensures each request $r_i \in \mathcal{R}$ must be picked up and dropped off by same route $m \in \mathcal{M}$, where $p_i$ and $d_i$ denote the pickup and dropoff locations for the request $r_i \in \mathcal{R}$. 

Next, we look into the constraints that ensure the assignments do not violate any time-related constraints.
The \cref{eqn:time_limit_constraint} ensures that, in route $m \in \mathcal{M}$, when a vehicle is assigned to move from node $i \in \mathcal{N}$ to node $j \in \mathcal{N}$, the vehicle can not reach node $j$ earlier than the minimum travel time $T_{i,j}$ between the nodes $i,j \in \mathcal{N}$ and additional dwell time $T_{d}$ (dwell time) for dropoff/pickup of passengers at the node $i$. The \cref{eqn:time_limit_constraint_f_start,eqn:time_limit_constraint_f_end} ensure that route $m \in \mathcal{M}$ when assigned vehicle  moving to node $j \in \mathcal{N}$ from the node $i \in \mathcal{N}$ satisfy the time constraints. 
 The \cref{eqn:pick_up_time_window,eqn:drop_off_time_window} ensures that all the nodes satisfy the time window constraints, where $\tau_s$ denote the allow slack time in the dropoff of the passengers. 
The \cref{eqn:operation_constraint_t_short} ensures that the total duration for the routes ($m \in \mathcal{M}$) does not exceed  $\tau_{max}$. 

Now, we look into the constraints that ensure the assignments do not violate any capacity-related constraints. The \cref{eqn:capacity_constraint_a,eqn:capacity_constraint_b,eqn:capacity_constraint_ss} ensure each route $m \in \mathcal{M}$ can only accommodate passengers based on the capacity of the assigned vehicle. Each pick-up point adds capacity equal to the total passenger capacity of the corresponding request to the vehicle. Each drop-off point reduces the current passengers in the vehicle by the total passenger capacity of the corresponding request. 



\paragraph{Objective}
We define the \emph{SchedulingObjective} which minimizes the cost of the scheduling requests to the routes and scheduling the routes to the vehicles.

\begin{itemize}
\item the total travel time of routes; 
\item the number of routes.
\end{itemize}

We can formally express the \emph{SchedulingObjective} as follows,

minimize:
{\scriptsize
\begin{align}
& W_1 \cdot \sum_{m \in \mathcal{M}}
(e^m - s^m) + W_2 \cdot |\mathcal{M}|
\label{eqn:scheduling}
\end{align}
} 





==> sub/linearization.tex <==
\subsection{Linearization of Constraints for Integer Programming}

\paragraph{Indicator variable}

\begin{itemize}
    \item $I_z^{min} \in\{0,1\}$ - If the duration is less than $\tau^{threshold}_{min}$, then $I_z^{min} = 0$, otherwise $I_z^{min} = 1$.
\end{itemize}

\subsubsection{Time Constraints}
 We can linearize the constraints in \cref{eqn:time_limit_constraint,eqn:time_limit_constraint_f_start,eqn:time_limit_constraint_f_end} as follows
    
    \begin{align}
        t^{i} - t^{j}  + T(i, j) + T_{dwell} \leq \left(1 - \sum_{m \in \mathcal{M}} x^z_{ij}\right) K_\infty \;\;\;\;\forall{i \in \mathcal{N}} \;\; \forall{j \in \mathcal{N}}
       \label{eqn:time_limit_constraint_linearized_ax}
    \end{align}

    \begin{align}
         f_z^{start} - t^j + T(i,j)  \leq \left(1 - x^z_{ij}\right) K_\infty \;\;\;\; \forall{i \in \mathcal{N}} \;\;\;\; \forall{j \in \mathcal{N}} \;\;\;\; \forall m \in \mathcal{M}
       \label{eqn:operation_constraint_1_linearized_ax}
    \end{align}
    
    \begin{align}
         t^i + T(i,j) + T_{dwell} - f_z^{end}  \leq \left(1 - x^z_{ij}\right) K_\infty \;\;\;\; \forall{i \in \mathcal{N}} \;\;\;\; \forall{j \in \mathcal{N}} \;\;\;\; \forall m \in \mathcal{M}
       \label{eqn:operation_constraint_2_linearized_ax}
    \end{align}
    
    
    where $K_\infty$ is a large constant.

    
    \paragraph{Duration Constraint}
\begin{itemize}
    \item Each run $m \in \mathcal{M}$ satisfy the following duration constraint.
        \begin{align}
         f_z^{end} - f_z^{start} - K_\infty \cdot  I_z^{min} \leq \tau^{threshold}_{min} \;\;\;\; \forall m \in \mathcal{M}
       \label{eqn:indicator_constraint_min}
    \end{align}
    
\end{itemize}

    
\subsubsection{Capacity Constraints}

    We can linearize the constraints in the \cref{eqn:capacity_constraint_a,eqn:capacity_constraint_b} as follows,
    \Aron{let's restrict $i$ to locations from which there is an edge to $p^j$ or $d^j$}    
    \begin{align}
        c^{i} -  c^{p^j} + n_j \leq \left(1 - \sum_{m \in \mathcal{M}} x^z_{ij}\right) K_\infty\;\;\;\;\forall{i \in \mathcal{N}}\;\;\;\;\forall{r_j \in \mathcal{R}}\\
        c^{i} -  c^{d^j} - n_j \leq \left(1 - \sum_{m \in \mathcal{M}} x^z_{ij}\right) K_\infty\;\;\;\;\forall{i \in \mathcal{N}}\;\;\;\;\forall{r_j \in \mathcal{R}}\\
        % wc^{i} -  wc^{p^j} + wn_j \leq \left(1 - \sum_{m \in \mathcal{M}} x^z_{ij}\right) K_\infty\;\;\;\;\forall{i \in \mathcal{N}}\;\;\;\;\forall{r_j \in \mathcal{R}}\\
        % wc^{i} -  wc^{d^j} - wn_j \leq \left(1 - \sum_{m \in \mathcal{M}} x^z_{ij}\right) K_\infty\;\;\;\;\forall{i \in \mathcal{N}}\;\;\;\;\forall{r_j \in \mathcal{R}}
    \end{align}
    
    
    

    where $K_\infty$ is a large constant.

\subsubsection{Operational Constraints}

We can linearize the constraints in \cref{eqn:operation_constraint_t_short} as follows
 
% Approach 01:
\begin{align}
f_z^{start} + \tau^{duration}_{min} - f_z^{end} \leq \left(1 - \sum_{v \in \mathcal{V}} e^v_z \right) K_\infty \;\;\;\; \forall{m \in \mathcal{M}}
\label{eqn:operation_constraint_t_short_min_linearized_a1}
\end{align}


\begin{align}
f_z^{end} - f_z^{start}  -  \tau^{duration}_{max}  \leq \left(1 - \sum_{v \in \mathcal{V}} e^v_z \right) K_\infty \;\;\;\; \forall{m \in \mathcal{M}} 
\label{eqn:operation_constraint_t_short_max_linearized_a2}
\end{align}
 


% Approach 02, By introducing new indicator variable $I^{type}_{z} \in \{0, 1\}$.
% \begin{align}
% f_z^{start} + \tau^{short}_{min} - f_z^{end} \leq \left(1 - \sum_{v \in \mathcal{V}} e^v_z \right) K_\infty \;\;\;\; \forall{m \in \mathcal{M}}
% \label{eqn:operation_constraint_t_short_min_linearized_ap2}
% \end{align}


% \begin{align}
% f_z^{end} - f_z^{start}  -  \tau^{short}_{max} - K_z \cdot I^{type}_{z} \leq \left(1 - \sum_{v \in \mathcal{V}} e^v_z \right) K_\infty \;\;\;\; \forall{m \in \mathcal{M}} 
% \label{eqn:operation_constraint_t_short_max_linearized_ap2}
% \end{align}
% where $K_z$ is a large constant.
    
% \begin{align}f_z^{end} - f_z^{start}  - \tau^{normal}_{max}  < \left(1 - \sum_{v \in \mathcal{V}} e^v_z \right) K_\infty \;\;\;\; \forall{m \in \mathcal{M}} \end{align}


% Approach 03,
% Simply introducing new variable $f^{duration} = f^{end} - f^{start}$
% \begin{align}
% \tau^{short}_{min} \leq f_z^{duration} < \tau^{short}_{max}
% \end{align}


% \begin{align}
% f_z^{duration} - \tau^{short}_{max} - K_z \cdot I^{type}_{z} \leq \left(1 - \sum_{v \in \mathcal{V}} e^v_z \right) K_\infty \;\;\;\; \forall{m \in \mathcal{M}_{short}} 
% \label{eqn:operation_constraint_t_short_max_linearized_ap3}
% \end{align}

We can linearize the constraint in \cref{eqn:operational_constraint_t_buffer} as follows
 

\begin{align}
f_{z_i}^{end} + \tau_{buffer} - f_{z_j}^{start} \leq \left(2 - e^v_{z_i} - e^v_{z_j} \right) K_\infty \;\;\;\; \forall{v \in \mathcal{V}}  \;\;\;\; \forall{z_i, z_j \in \mathcal{Z}}
\end{align}

where $K_\infty$ is a large constant.




\subsection{Linearization of Objective for Integer Programming}

We can simplify \cref{eqn:obj_part_01}, by introducing three additional variables $m^z \in \mathbb{Z}^{+}$, ${m_1}^z \in \{0,1\}$, ${m_2}^z  \in \{0,1\}$. The variables ${m_1}^z$, ${m_2}^z$ are indicator variables that make the constraints into either active or inactive state.
\begin{align}
    \min(\tau^{threshold}_{min},  f^{end}_z - f^{start}_z)
    \label{eqn:obj_part_01}
\end{align}

Also, the newly added variables need to met the following constraints.
\begin{align*}
    m^z \geq \tau^{threshold}_{min} - K_\infty \cdot {m_1}^z  \;\;\;\; \forall{m \in \mathcal{M}}\\
    m^z \geq f^{end}_z - f^{start}_z - K_\infty \cdot {m_2}^z \;\;\;\; \forall{m \in \mathcal{M}}\\
    {m_1}^z + {m_2}^z = 1 \;\;\;\; \forall{m \in \mathcal{M}}\\
    0 \leq {m}^z \leq \tau^{threshold}_{min}   \;\;\;\; \forall{m \in \mathcal{M}}\\
\end{align*}


Similarly, we can simplify \cref{eqn:obj_part_04}, by introducing three additional variables $g^z \in \mathbb{Z}^{+}$, ${g_1}^z \in {0,1}$, ${g_2}^z  \in {0,1}$. The variables ${g_1}^z$, ${g_2}^z$ are indicator variables that make constraints into either active or inactive state.
\begin{align}
\min\left\{1, \sum_{m \in \mathcal{M}} e^v_z\right\}
    \label{eqn:obj_part_04}
\end{align}

Again, the newly added variables need to met the following constraints.
\begin{align*}
    g^v \geq 1 - K_\infty \cdot {g_1}^z  \;\;\;\; \forall{v \in \mathcal{V}}\\
    g^v \geq \sum_{m \in \mathcal{M}} e^v_z - K_\infty \cdot {g_2}^z \;\;\;\; \forall{v \in \mathcal{V}}\\
    {g_1}^v + {g_2}^v = 1 \;\;\;\; \forall{v \in \mathcal{V}}\\
    0 \leq g^v \leq 1 \;\;\;\; \forall{v \in \mathcal{V}}
\end{align*}


Finally, we can simplify \cref{eqn:obj_part_03}, by introducing additional variable $o^z \in \mathbb{Z}^{+}$.
\begin{align}
\max\left\{0,  f^{end}_z - f^{start}_z - \tau^{threshold}_{max}\right\}
    \label{eqn:obj_part_03}
\end{align}

Again, the newly added variable need to met the following constraints.
\begin{align*}
    o^z \geq f^{end}_z - f^{start}_z -  \tau^{threshold}_{max} \;\;\;\; \forall{m \in \mathcal{M}}\\
       0 \leq o^z < \tau^{normal}_{max} - \tau^{threshold}_{max} \;\;\;\; \forall{m \in \mathcal{M}}
\end{align*}


==> sub/real_time_model.tex <==
% \paragraph{Real-time Problem Model}
% The real-time problem focus on determining the optimal narrow pick-up time window from a broader time window ([$A^i, B^i$]) requested by user request.

% For the real-time problem, we assume that every user request $r_i \in \mathcal{R}$ comes to the system by following a uniform distribution during previous day when the system receives calls from users. We model distribution of the pickup location and broader pick-up window as a machine learning model $K(h_{p_i}, h_{d_i}, t_i, w_i)$ that predicts the how a particular time is busy based on $t_i \in \mathbb{Z}^{+}, w_i \in \mathcal{W}$ when assigning request from the pickup zone $h_{p_i} \in \mathcal{H}$ to dropoff zone $h_{d_i} \in \mathcal{H}$, where $\mathcal{W}$ indicates the set of the day of week, and $\mathcal{H}$ indicates the set of geographical zones.

% Further, to express the simply we introduce few additional notations. We denote the graph before the including of the new request $r_i$ as $G^{{r_i}^{-}}$, and the graph after the including the new request $r_i$ as $G^{{r_i}^{+}}$. Similarly, we denote the set of nodes that present in the graph before the including the new request $r_i$ as $\mathcal{N}^{{r_i}^{-}}$, and the nodes that presents after including the new request $r_i$ as $\mathcal{N}^{{r_i}^{+}}$. We assume that there are enough vehicles ($\mathcal{V}$) and routes ($\mathcal{M}$) present in the system to serve all the requests.

% \paragraph{Decision Variables} We add the following additional decision variables in the real-time problem model. $a^{i} \in \mathbb{Z}^{+}$ --- indicates the earliest pick-up time for the request $r_i \in \mathcal{R}$. $b^{i} \in \mathbb{Z}^{+}$ --- indicates the latest pick-up time for the request $r_i \in \mathcal{R}$.

% \paragraph{Constraints} The real-time problem model needs to ensure the following additional constraint in addition to the constraints mentioned for the extended PDPTW model.

% \begin{align}
%     A^i \leq a^i <  b^i \leq B^i \;\;\;\; \forall {r_i \in \mathcal{R}}
%     \label{eqn:new_request}
% \end{align}

% The \cref{eqn:new_request} ensures that the narrow time window should be within the range of the broader time window.

% Whenever a new request $r_i \in \mathcal{R}$ comes to the system, we define the current state of the system by following set of inputs,

% \begin{align*}
%     r_i : {p_i, d_i, [A^i, B^i], c_i}\\
%     \mathcal{S}_{\mathcal{R}^{{r_i}^{-}}},  BN(h_{p_i}, h_{d_i}, t_i, w_i)
% \end{align*}




